Gaussian Variational Schemes on Bounded and Unbounded Domains

A machine-learnable variational scheme using Gaussian radial basis functions (GRBFs) is presented and used to approximate linear problems on bounded and unbounded domains. In contrast to standard mesh-free methods, which use GRBFs to discretize strong-form differential equations, this work exploits the relationship between integrals of GRBFs, their derivatives, and polynomial moments to produce exact quadrature formulae which enable weak-form expressions. Combined with trainable GRBF means and covariances, this leads to a flexible, generalized Galerkin variational framework which is applied in the infinite-domain setting where the scheme is conforming, as well as the bounded-domain setting where it is not. Error rates for the proposed GRBF scheme are derived in each case, and examples are presented demonstrating utility of this approach as a surrogate modeling technique.

==> 09-whitney-deprecated.tex <==
\section{Application: Whitney Forms and Exterior Calculus in High Dimensions}
\label{sec:whitney}

The final example presented here involves the use of Whitney $k$-forms, which are finite-dimensional differential $k$-forms on a simplicial complex \cite{lohi2021whitney} useful in building compatible discretizations and faithful representations of the de Rham complex corresponding to a PDE system \cite{trask2020conservative, bochev2007principles}. Building surrogate models using Whitney forms is of particular interest due to difficulties with the maintenance of underlying structure, such as geometric invariants, in traditional surrogate modeling techniques \cite{berry2020spectral, gruber2023energetically, actor2024data}.  The GRBF methods developed here are particularly attractive for this task, since other machine-learning approaches for learning Whitney forms, e.g., \cite{actor2024data}, scale poorly with dimension, making them impractical for many real-world applications.


% % traditional surrogate modeling techniques to maintain the geometric invariants and underlying structure of the underlying PDE system \cite{berry2020spectral, gruber2023energetically, actor2024data}. 
% Other machine-learning approaches for learning Whitney forms \cite{actor2024data} scale poorly with dimension, making them impractical for many real-world applications.

% We briefly review key details regarding exterior calculus, Whitney forms, and their role in data-driven surrogates models, before describing how to build Whitney forms in our GRBF scheme.

% \subsection{Exterior Calculus and Whitney Forms}

To describe how Whitney's construction works, recall the notion of a chain complex on the graded vector space $V=\bigoplus_{k=-\inf}^{\inf}V_k$, which is a sequence of vector subspaces $V_k$ along with linear maps $\partial_k:V_k\to V_{k-1}$ satisfying $\partial_{k+1}\circ\partial_k = 0$, i.e., $\mathrm{im}\,\partial_k \subseteq \mathrm{ker}\,\partial_{k+1}$.  These $V_k$ spaces are commonly chosen as the spaces of $k$-simplices that discretize a domain $\Omega$, and $\partial_k$ is taken to be the boundary operator taking a simplicial chain $v_k\in V_k$ to its boundary chain $\partial v_k\in V_{k-1}$ of one degree lower. The topological duals of the $\partial_k$ under the standard integration pairing, denoted by $d_k:V_k^*\to V_{k+1}^*$, are the exterior derivatives, which are defined so that Stokes' theorem holds:  for any simplex $v\in V^k$ and differential $k$-form  $\omega\in\Lambda^k$,
\[\int_{\partial v}\omega = \int_v d\omega.\]
Importantly, it follows that $d_k\circ d_{k-1}=0$, a property which must be respected by any discretization of the spaces $V_k^*$.  Note that $d_0,d_1,d_2$ are the abstract analogues of the usual vector calculus operators $\nabla, \nabla\times, \nabla\cdot$ defined so that $\nabla\times\nabla = \nabla\cdot\nabla\times = 0$.

% Stokes' theorem, expressed 
% for a simplex $v\in V^k$ and a differential $k$-form  $\omega\in\Lambda^k$ as
% \[\int_{\partial v}\omega = \int_v d\omega,\]
% then induces a dual cochain complex in terms of
% the coboundary operators $d_k:V^k\to V_{k+1}$, which are restrictions of the exterior derivative to $k$-forms on $V_k$:

% \ANT{TikZ picture here}

% The spaces $\lambda^k$ can be consistently discretized with Whitney $k$-forms,
Remarkably, Whitney $k$-forms yield a compatible discretization of $V_k^*$ and are defined as follows: for any simplex $v = [p_0,...,p_k] \in V_k$, 
\begin{align*}
    W_v = k! \sum_{i=0}^k (-1)^i \lambda_i \, d\lambda_0\wedge...\wedge\widehat{d\lambda_i}\wedge...\wedge d\lambda_k,
\end{align*}
where $\lambda_i:V_k\to\mathbb{R}$ are the barycentric coordinates and $\widehat{d\lambda_i}$ indicates a term which is left out.  It follows that $d_{k+1}\circ d_k = 0$ for all Whitney forms $\mathcal{W}_v$, as required for de Rham compatibility.  Moreover, the Whitney $k$-forms contain all constant $k$-forms since they form a partition of unity, i.e. $\sum\lambda_i(~x)=1$ for all $~x$.  In the context of machine-learned surrogate models, such barycentric coordinates or partitions of unity can come from a coarsened graph representation of the domain \cite{trask2022enforcing} or otherwise calibrated based on data \cite{actor2024data} to provide a basis that matches data from high-fidelity simulations. 

% Importantly, the use of Whitney forms ensures that consequences of the cochain complex are exactly preserved, enabling reconstructions which preserve involution constraints and are free of spurious computational modes. In the context of this work, we use GRBFs to define the spaces $V^k$, taking care to preserve the properties of the underlying chain complex.

% There are two essential ingredients: first, there is the use of Gaussian RBFs as Whitney $k$-forms, which leads to the spatial compatibility necessary for an effective mixed method.  Second, there is the treatment of boundaries, which nonobvious due to the use of noncompactly supported RBFs.  

% \subsection{Using Gaussian RBFs as Whitney \texorpdfstring{$k$}-Forms}
% \label{sec:whitney-ex}

% \begin{itemize}
% \item discussion of compatibility of using Gaussians, since no POU property
% \item add $\mathbf{1}$ to basis
% \end{itemize}

While the proposed GRBF basis functions do not form a partition of unity, they can still be used to build Whitney forms.  Defining the constant function $\phi_0(~x)=1$, the set $\{\phi_0,\dots,\phi_n\}$ form a Whitney 0-form basis for functions on $\mathbb{R}^d$, from which a vector proxy for the Whitney 1-forms can be constructed as
\begin{align*}
    \psi_{ij}(~x) &= \phi_i(~x)\nabla\phi_j(~x)-\phi_j(~x)\nabla\phi_i(~x) = \phi_i(~x)\phi_j(~x)\lr{~p_j(~x)-~p_i(~x)},
    % \psi_{ij}(~x) &= \phi_i(~x)\nabla\phi_j(~x)-\phi_j(~x)\nabla\phi_i(~x) = \phi_i(~x)\phi_j(~x)\lr{~C^{-1}_i(~x-~m_i)-~C^{-1}_j(~x-~m_j)},
\end{align*}
where $0\leq i<j\leq n$ and $~m_0, ~C_0^{-1}$ are treated as identically zero.  Clearly, the anticommutative relationship $\psi_{ji}=-\psi_{ij}$ holds for all pairs of indices $i,j$, as required for a 1-form basis.  Moreover, it follows that the nontrivial gradient of each 0-form is expressible as
\[\nabla\phi_i(~x) = \phi_0(~x)\nabla\phi_1(~x)-\phi_1(~x)\nabla\phi_0(~x) = \psi_{01},\]
so that the gradient of each 0-form is contained in the span of the 1-form basis.  \ANT{This ensures that ...  }

It is straightforward to check that this relationship persists for higher-order $k$-forms.  More precisely, considering a simplex $v = [p_{i_0},...,p_{i_k}]$ and using the fact that $d\phi_i(~x) = \phi_i(~x)~p_i(~x)\cdot d~x$, it follows that
\begin{equation*}
    W_v = k!\prod_{j=0}^k \phi_{i_j} \sum_{j=0}^k \lr{-1}^j \lr{~p_{i_0}\cdot d~x}\wedge ...\wedge \widehat{~p_{i_j}\cdot d~x}\wedge ... \wedge \lr{~p_{i_k}\cdot d~x},
\end{equation*}
so that the same product of Gaussian PDFs appears in every term. 

% \ANT{probably should state general formula}

\begin{remark}
    The nonstandard inclusion of the constant function $\phi_0=1$ in the 0-form basis is present because Gaussian RBFs do not form a partition of unity.  Since nonzero constants are not integrable on infinite domains, this requires some conceptual modification for this case \ANT{need to address this}
\end{remark}


Before moving to some numerical examples, we present a few corollaries which illustrate how Theorem~\ref{thm:quadrature} appears in important special cases.  For comparison, direct calculations of these expressions by a different method are given in Appendix~\ref{app:handcalc}. \JONAS{We haven't introduced the problem we want to solve, so $M^1$, etc. are all undefined}

\begin{corollary}
The mass matrix $~M^0$ of 0-forms and stiffness matrix $~S^0$ of 0-form gradients are given component-wise as 
\begin{equation*}
    M^0_{ij} = \intIP{\psi_i}{\psi_j} = I^{2,0}_{ij}, \qquad S^0_{ij} = \intIP{\nabla\psi_i}{\nabla\psi_j} = \tr \left( ~I^{0,2}_{ij} \right).
\end{equation*}
Additionally, the mixed matrix $~V^0$ between 0-form gradients and 1-forms is given component-wise as
\begin{equation*}
    V^0_{i,ab} = \intIP{\nabla\psi_i}{\psi_{ab}} = \tr\lr{~I^{1,2}_{a,bi}-~I^{1,2}_{b,ai}}.
\end{equation*}
\end{corollary}

\begin{corollary}\label{cor:1formM}
The mass matrices $~M^1$ of 1-forms and $~M^2$ of 2-forms are given component-wise as 
\begin{align*}
    M^1_{ij,ab} &= \intIP{\psi_{ij}}{\psi_{ab}} = \tr \left( ~I^{2,2}_{ia,jb} - ~I^{2,2}_{ib,ja} - ~I^{2,2}_{ja,ib} + ~I^{2,2}_{jb,ia} \right), \\
    M^2_{ijk,abc} &= \intIP{\psi_{ijk}}{\psi_{abc}} = \sum_{(ijk)} \sum_{(abc)} \tr_{12} \tr_{34} \left( ~{I}^{2,4}_{ia,jbkc} - ~{I}^{2,4}_{ia,jckb} \right),
\end{align*}
where $\tr_{ij}$ denotes a trace over indices $i,j$ in its tensor argument.  Moreover, the mixed matrix between 1-form curls and 2-forms is given component-wise as
\begin{equation*}
    ~V^1_{ij,abc} = \intIP{\nabla \times \psi_{ij}}{\psi_{abc}} = 2 \sum_{(abc)} \tr_{12}\tr_{34}\left( ~I^{1,4}_{a,ibjc} - ~I^{1,4}_{a,icjb} \right).
\end{equation*}
\end{corollary}

% \begin{corollary}
% The mixed matrix between 0-forms and 1-forms $\mathbf{V}^0$ is given as $$\mathbf{V}^0_{i,ab} = \langle \nabla \psi_i, \psi_{ab} \rangle = \tr \left( \mathbf{I}^{1,2}_{a,bi}  - \mathbf{I}^{1,2}_{b,ai}\right).$$
% \end{corollary}
% % \color{red}{
% \begin{corollary}
% The mixed matrix between 1-forms and 2-forms $\mathbf{V}^1$ is given as $$\mathbf{V}^1_{ij,abc} = \langle \nabla \times \psi_{ij}, \psi_{abc} \rangle = 2 \sum_{(abc)} \tr \left( \tr \left( \mathbf{I}^{1,4}_{a,ibjc} - \mathbf{I}^{1,4}_{a,icjb} \right) \right) .$$
% \end{corollary}
\begin{corollary}
When we add the function $\mathbf{1}$ into our 1-form basis construction, in our competed space of 1-forms $\widehat{V}^1$, the mass matrix of 1-forms $\widehat{\mathbf{M}}^1$ becomes
$$ \widehat{\mathbf{M}}^1 = \begin{bmatrix} \mathbf{S}^0 & {\mathbf{V}^0} \\ {\mathbf{V}^0}^T & \mathbf{M}^1 \end{bmatrix},$$
and the mixed matrix $\widehat{\mathbf{V}}^0$ becomes
$$ \widehat{\mathbf{V}}^0 = \begin{bmatrix} \mathbf{S}^0 & {\mathbf{V}^0} \end{bmatrix}.$$
Similar expressions can be constructed for $\widehat{\mathbf{M}}^2,\,\widehat{\mathbf{V}}^1$, etc.
\end{corollary}
% }\color{black}

% For $\ell=1,\dots,L$, let $X_\ell \sim \mathcal{N}(\mathbf{m}_\ell, \mathbf{C}_\ell)$ be a Gaussian distribution in $\mathbb{R}^n$, with a corresponding probability distribution function $\phi_\ell$.


% Consider the tensor $\mathbf{I}^{\alpha,\beta}_{i_1,\dots,i_\alpha;j_1,\dots,j_\beta}$ of size $n^{\otimes \beta}$ defined by

% Let $~X$ and $Z$ be the Gaussian random variable and the corresponding normalization constant given by Lemma \ref{lem:gaussprod} for the product of Gaussians $\left( \prod_{a=1}^\alpha \phi_{i_a} \right) \cdot \left( \prod_{b=1}^\beta \phi_{j_b} \right)$, and let $\mathbf{M}^k = \mathbb{E}(\mathbf{X}^{\otimes k}).$
% Then,
% \begin{equation}
% \mathbf{I}^{\alpha,\beta}_{i_1,\dots,i_\alpha; j_1,\dots,j_\beta} = Z \left( \bigotimes_{b=1}^\beta \mathbf{C}_{j_b}^{-1} \right) \times_E \left( \sum_{k=0}^\beta \sum_{\substack{\vec{j} \in 2^{\lvert \beta \rvert} \\ \lvert \vec{j} \rvert = k}} (-1)^{\beta-k} \left( \bigotimes_{b=1}^k \mathbf{m}_{j_b} \otimes \mathbf{M}^{\beta-k} \right)_{\sigma_{\vec{j}}} \right),
% \end{equation}

% Therefore, the 1-form mass matrix entry $\mathcal{~M}_{ij,ab}$ for $0<i,a<j,b$ can be approximated as
% \begin{align*}
%     \mathcal{M}_{ij,ab} &= \int_\Omega \psi_{ij}\cdot\psi_{ab} \approx \int_{\mathbb{R}^d}\psi_{ij}\cdot\psi_{ab} \\
%     &= \int_{\mathbb{R}^d} \phi_i(~x)\phi_j(~x)\phi_a(~x)\phi_b(~x)\lr{~C^{-1}_i(~x-~m_i)-~C^{-1}_j(~x-~m_j)}\cdot\lr{~C^{-1}_a(~x-~m_a)-~C^{-1}_b(~x-~m_b)} \\
%     &= z_{ijab}\int_{\mathbb{R}^d} \phi_{ijab}(~x)\lr{~C^{-1}_i(~x-~m_i)-~C^{-1}_j(~x-~m_j)}\cdot\lr{~C^{-1}_a(~x-~m_a)-~C^{-1}_b(~x-~m_b)} \\
%     &= z_{ijab}\,\mathbb{E}\left[\lr{~C^{-1}_i(~x-~m_i)-~C^{-1}_j(~x-~m_j)}\cdot\lr{~C^{-1}_a(~x-~m_a)-~C^{-1}_b(~x-~m_b)}\right].
% \end{align*}
% Note that the approximation error decays exponentially with the covariances $~C_i$ and can be made arbitrarily small by adjusting this parameter \ANT{double check this}.  It follows that all integrals necessary for the scheme can be approximated as polynomial moments, computed with the formulae proven in Appendix~\ref{app:someting}. \ANT{mention something about curse of dimensionality?}


==> 98-purgatory.tex <==
% \section{Implementation}
% \label{sec:implementation}


% \subsection{Implementation by Polynomial Moments}

% For a vector $\mathbf{x} \in \mathbb{R}^n$, denote $\mathbf{x}^{\otimes d} := \mathbf{x} \otimes \mathbf{x} \otimes \cdots \otimes \mathbf{x}$ be the outer (tensor) product of $\mathbf{x}$ against itself $d$ times.
% From \cite{pereira2022tensor}, we have the following lemma.
% \begin{lemma} (From \cite{pereira2022tensor})
% Let $X \sim \mathcal{N}(\mathbf{m}, \mathbf{C})$. Then,
% \begin{equation}
% \mathbb{E}( X^{\otimes d} ) = \int_{\mathbb{R}^n} \mathbf{x}^{\otimes d} \, \mathbb{P}(X = \mathbf{x}) d\mathbf{x} = \sum_{k=0}^{\left \lfloor d/2 \right \rfloor} C_{d,k} \text{sym}\left( \mathbf{m}^{\otimes(d-2k)} \otimes \mathbf{C}^{\otimes k} \right), 
% \end{equation}
% where $$C_{d,k} = \begin{pmatrix} d \\ 2k \end{pmatrix} \frac{ (2k)! }{k! 2^k}.$$
% \label{lem:gaussian_moment}
% \end{lemma}
% Note that when $d=2$, this reduces to \Cref{lem:cov}.


% In the spirit of \cite{bader2006algorithm}, define the \textit{even-modal tensor product} $\times_E$ as follows: for tensor $A$ of size $n_1 \times n_2 \times \cdots \times n_{2p}$ and $B$ of size $ n_2 \times n_4 \times n_6 \times \cdots \times n_{2p}$, the even-mode tensor product $A \times_E B$ is given as $$ (A \times_E B)_{i_1,\dots,i_{2p-1}} = \sum_{i_2} \sum_{i_4} \cdots \sum_{i_{2p}} A_{i_1,i_2,\dots,i_{2p}} B_{i_2,i_4,i_6\dots,i_{2p}}. $$
% Using Lemma \ref{lem:gaussian_moment}, we have the following result:

% \begin{proof}[Proof of Proposition~\ref{prop:main}]
% By the definition of the gradient of Gaussian functions, 
% \begin{equation*} \begin{split}\left( \prod_{a=1}^\alpha \phi_{i_a}(\mathbf{x}) \right) \left( \bigotimes_{b=1}^\beta \nabla \phi_{j_b}(\mathbf{x}) \right)
% &= \left( \prod_{a=1}^\alpha \phi_{i_a}(\mathbf{x}) \right) \left( \prod_{b=1}^\beta \phi_{j_b}(\mathbf{x}) \right)  \left( \bigotimes_{b=1}^\beta \mathbf{C}_{j_b}^{-1}\left( \mathbf{m}_{j_b} - \mathbf{x} \right) \right) \\
% &= Z \Phi(\mathbf{x})  \left( \bigotimes_{b=1}^\beta \mathbf{C}_{j_b}^{-1}\left( \mathbf{m}_{j_b} - \mathbf{x} \right) \right) \\
% \end{split} \end{equation*}
% where $\Phi$ is the probability distribution function for $\mathbf{X}$.
% Integrating the above expression, it follows that
% \begin{equation*} \begin{split}
% \mathbf{I}^{\alpha,\beta}_{i_1,\dots,i_\alpha;j_1,\dots,j_\beta} 
% &= Z \, \mathbb{E} \left[ \bigotimes_{b=1}^\beta \mathbf{C}_{j_b}^{-1}(\mathbf{m}_{j_b} - \mathbf{X} ) \right] \\
% &= Z \, \left( \bigotimes_{b=1}^\beta \mathbf{C}_{j_b}^{-1} \right) \times_E \mathbb{E}\left[ \bigotimes_{b=1}^\beta ( \mathbf{m}_{j_b} - \mathbf{X}) \right],
% \end{split} \end{equation*}
% where the expectation is taken over the random variable $\mathbf{X}$.
% We expand the outer product inside the expectation into each of its constituent terms; each of these terms has a number of modes resulting from outer products involving $\mathbf{X}$, and the remaining modes consist of means $\mathbf{m}_{j_b}$. In this expansion, we then group terms by the number of $\mathbf{X}$'s that appear in each expression. Denote the number of means $\mathbf{m}_{j_b}$ that appear as $k$, and thus the number of appearances of $\mathbf{X}$'s (i.e. the moment of $\mathbf{X}$ that needs to be computed in each term) is $\beta-k$.
% As a result,
% \begin{equation*}
% \mathbb{E}\left[ \bigotimes_{b-1}^\beta (\mathbf{m}_{j_b} - \mathbf{X}) \right] = \mathbb{E} \left[ \sum_{k=0}^\beta \sum_{\substack{\vec{j} \in 2^{\lvert \beta \rvert} \\ \lvert \vec{j} \rvert = k}} (-1)^{\beta-k} \left( \left( \bigotimes_{b=1}^k \mathbf{m}_{j_b} \right) \otimes \mathbf{X}^{\otimes (\beta-k)} \right)_{\sigma_{\vec{j}}} \right].
% \end{equation*}
% By linearity of expectation,
% \begin{equation*} \begin{split}
% \mathbb{E}\left[ \bigotimes_{b=1}^\beta (\mathbf{m}_{j_b} - \mathbf{X}) \right] 
% &= \sum_{k=0}^\beta \sum_{\substack{\vec{j} \in 2^{\lvert \beta \rvert} \\ \lvert \vec{j} \rvert = k}} (-1)^{\beta-k} \left( \left( \bigotimes_{b=1}^k \mathbf{m}_{j_b} \right) \otimes \mathbb{E} \left[  \mathbf{X}^{\otimes (\beta-k)} \right] \right)_{\sigma_{\vec{j}}} \\
% &= \sum_{k=0}^\beta \sum_{\substack{\vec{j} \in 2^{\lvert \beta \rvert}\\ \lvert \vec{j} \rvert = k}} (-1)^{\beta-k} \left( \left( \bigotimes_{b=1}^k \mathbf{m}_{j_b} \right) \otimes \mathbf{M}^{\beta-k}  \right)_{\sigma_{\vec{j}}}.
% \end{split} \end{equation*}
% % where $2^{\lvert \beta \rvert}$ is the power set of the set $\{1,\dots,\beta \}$; $\vec{j}$ is a multi-index representing a subset of the power set $2^{\lvert \beta \rvert}$; and $\sigma_{\vec{j}}$ is the unique permutation of $\beta$ elements that maps the first $k = \lvert \vec{j} \rvert$ elements to positions $j_1,\dots,j_k$, and the rest of the elements \textit{in order} to positions $j_{k+1},\dots,j_\beta$.
% Therefore,
% \begin{equation}
% \mathbf{I}^{\alpha,\beta}_{i_1,\dots,i_\alpha; j_1,\dots,j_\beta} = Z \left( \bigotimes_{b=1}^\beta \mathbf{C}_{j_b}^{-1} \right) \times_E  \left(  \sum_{k=0}^\beta \sum_{\substack{\vec{j} \in 2^{\lvert \beta \rvert} \\ \lvert \vec{j} \rvert = k}} (-1)^{\beta-k} \left( \left(  \bigotimes_{b=1}^k \mathbf{m}_{j_b} \right) \otimes \mathbf{M}^{\beta-k} \right)_{\sigma_{\vec{j}}} \right).
% \end{equation}


% \end{proof}
% \begin{corollary}
% The mass matrix of 0-forms $\mathbf{M}^0$ is given as $$\mathbf{M}^0_{ij} = \langle \psi_i, \psi_j \rangle = \mathbf{I}^{2,0}_{ij}.$$
% \end{corollary}
% \begin{corollary}
% The stiffness matrix of 0-forms $\mathbf{S}^0$ is given as $$\mathbf{S}^0_{ij} = \langle \nabla \psi_i, \nabla \psi_j \rangle = \tr \left( \mathbf{I}^{0,2}_{ij} \right).$$
% \end{corollary}
% \begin{corollary}
% The mass matrix of 1-forms $\mathbf{M}^1$ is given as $$\mathbf{M}^1_{ij,ab} = \langle \psi_{ij}, \psi_{ab} \rangle =  \tr \left( \mathbf{I}^{2,2}_{ia,jb} - \mathbf{I}^{2,2}_{ib,ja} - \mathbf{I}^{2,2}_{ja,ib} + \mathbf{I}^{2,2}_{jb,ia} \right).$$
% \end{corollary}
% \begin{corollary}
% The mass matrix of 2-forms $\mathbf{M}^2$ is given as $$\mathbf{M}^2_{ijk,abc} = \langle \psi_{ijk}, \psi_{abc} \rangle = \sum_{(ijk)} \sum_{(abc)} \tr \left( \tr \left( \mathbf{I}^{2,4}_{ia,jbkc} - \mathbf{I}^{2,4}_{ia,jckb} \right) \right),$$
% where the two traces are taken over the first two and second two sets of modes, respectively. Note this matches the expression in \Cref{subsec:two-forms}.
% \end{corollary}
% \begin{corollary}
% The mixed matrix between 0-forms and 1-forms $\mathbf{V}^0$ is given as $$\mathbf{V}^0_{i,ab} = \langle \nabla \psi_i, \psi_{ab} \rangle = \tr \left( \mathbf{I}^{1,2}_{a,bi}  - \mathbf{I}^{1,2}_{b,ai}\right).$$
% \end{corollary}
% % \color{red}{
% \begin{corollary}
% The mixed matrix between 1-forms and 2-forms $\mathbf{V}^1$ is given as $$\mathbf{V}^1_{ij,abc} = \langle \nabla \times \psi_{ij}, \psi_{abc} \rangle = 2 \sum_{(abc)} \tr \left( \tr \left( \mathbf{I}^{1,4}_{a,ibjc} - \mathbf{I}^{1,4}_{a,icjb} \right) \right) .$$
% \end{corollary}
% \begin{corollary}
% When we add the function $\mathbf{1}$ into our 1-form basis construction, in our competed space of 1-forms $\widehat{V}^1$, the mass matrix of 1-forms $\widehat{\mathbf{M}}^1$ becomes
% $$ \widehat{\mathbf{M}}^1 = \begin{bmatrix} \mathbf{S}^0 & {\mathbf{V}^0} \\ {\mathbf{V}^0}^T & \mathbf{M}^1 \end{bmatrix},$$
% and the mixed matrix $\widehat{\mathbf{V}}^0$ becomes
% $$ \widehat{\mathbf{V}}^0 = \begin{bmatrix} \mathbf{S}^0 & {\mathbf{V}^0} \end{bmatrix}.$$
% Similar expressions can be constructed for $\widehat{\mathbf{M}}^2,\,\widehat{\mathbf{V}}^1$, etc.
% \end{corollary}
% % }\color{black}

% \subsection{Implementation via Gauss-Hermite Quadrature}
% While the analytic expressions presented in the above section are tractable (and can be sufficiently vectorized to be efficiently computed on a CPU), the complexity of the summations, symmetrizations, and permutations make this approach inefficient and unwieldy for computing on GPUs, which due to memory requirements thereby limits the effectiveness of this scheme during training. Thus, we also demonstrate how such integrals can be computed exactly using Gauss-Hermite quadrature, assuming enough quadrature points are taken to exactly integrate polynomials of sufficient order.

% \begin{lemma}
% For $\ell=1,\dots,L$, let $X_\ell \sim \mathcal{N}(\mathbf{m}_\ell, \mathbf{C}_\ell)$ be a Gaussian distribution in $\mathbb{R}^n$, with a corresponding probability distribution function $\phi_\ell$.
% Choose (with replacement) $\alpha+\beta$ indices from the set $\{1,\dots,L\}$, and denote these indices $i_1,\dots,i_\alpha,j_1,\dots,j_\beta$.

% Consider the tensor $\mathbf{I}^{\alpha,\beta}_{i_1,\dots,i_\alpha;j_1,\dots,j_\beta}$ of size $n^{\otimes \beta}$ defined by
% \begin{equation}
% \mathbf{I}^{\alpha,\beta}_{i_1,\dots,i_\alpha;j_1,\dots,j_\beta} = \int_{\mathbb{R}^n} \left( \prod_{a=1}^\alpha \phi_{i_a}(\mathbf{x}) \right) \left( \bigotimes_{b=1}^\beta \nabla \phi_{j_b}(\mathbf{x}) \right) \, d\mathbf{x}.
% \end{equation}
% Let $\mathbf{X}$ and $Z$ be the Gaussian random variable and the corresponding normalization constant given by Lemma \ref{lem:gaussprod} for the product of Gaussians $\phi = \left( \prod_{a=1}^\alpha \phi_{i_a} \right) \cdot \left( \prod_{b=1}^\beta \phi_{j_b} \right)$ with the distribution $\mathcal{N}(\mathbf{m}, \mathbf{C})$, and let 
% $\mathbf{y},\mathbf{\omega}$ be Gauss-Hermite quadrature nodes and weights, respectively, for polynomials of degree $\beta$, with a total of $N_\text{quad}$ quadrature points.
% Then,
% \begin{equation}
% \mathbf{I}^{\alpha,\beta}_{i_1,\dots,i_\alpha; j_1,\dots,j_\beta} =
% Z \, \pi^{-\frac{n}{2}}  \sum_{k=1}^{N_\text{quad}} \mathbf{\omega}_k \left( \bigotimes_{b=1}^\beta \mathbf{C}^{-1}_{j_{b}} \left(\mathbf{m}_{j_b} - \left( \sqrt{2} \mathbf{C}^{\frac{1}{2}} \mathbf{y}_k + \mathbf{m} \right) \right) \right),
% \end{equation}
% where $\mathbf{C}^{\frac{1}{2}}$ is the Cholesky factor of the covariance matrix $\mathbf{C}$.
% \end{lemma}
% \begin{proof}
% For simplicity, define the tensor-valued polynomial $$\mathbf{p}(\mathbf{x}) = \bigotimes_{b=1}^\beta \mathbf{C}^{-1}_{j_{b}} \left(\mathbf{m}_{j_b} - \mathbf{x} \right).$$
% By our product of Gaussians result,
% \begin{equation*}\begin{split}
% \mathbf{I}^{\alpha,\beta}_{i_1,\dots,i_\alpha;j_1,\dots,j_\beta} &= \int_{\mathbb{R}^n} \left( \prod_{a=1}^\alpha \phi_{i_a}(\mathbf{x}) \right) \left( \bigotimes_{b=1}^\beta \nabla \phi_{j_b}(\mathbf{x}) \right) \, d\mathbf{x} \\
% &= \int_{\mathbb{R}^n} \left( \prod_{a=1}^\alpha \phi_{i_a}(\mathbf{x}) \right) \left( \bigotimes_{b=1}^\beta \phi_{j_b}(\mathbf{x}) \right) \mathbf{p}(\mathbf{x}) \, d\mathbf{x} \\
% &= Z \int_{\mathbb{R}^n} \phi(\mathbf{x}) \mathbf{p}(\mathbf{x}) \, d\mathbf{x}.
% \end{split} \end{equation*}
% Expanding out the definition for the probability distribution function $\phi$, and then applying a change of variables $\widehat{\mathbf{x}} = \frac{1}{\sqrt{2}} \mathbf{C}^{-\frac{1}{2}}\left(\mathbf{x}-\mathbf{m}\right)$,
% \begin{equation*}\begin{split}
% \mathbf{I}^{\alpha,\beta}_{i_1,\dots,i_\alpha;j_1,\dots,j_\beta}
% &= Z \, \left(2 \pi\right)^{-\frac{n}{2}} \det(\mathbf{C})^{-\frac{1}{2}} \int_{\mathbb{R}^n} \exp \left(-\frac{1}{2}\left(\mathbf{x}-\mathbf{m}\right)^T \mathbf{C}^{-1}\left(\mathbf{x}-\mathbf{m} \right) \right) \mathbf{p}(\mathbf{x}) \, d\mathbf{x} \\
% &= Z \, \left(2 \pi\right)^{-\frac{n}{2}} \det(\mathbf{C})^{-\frac{1}{2}} \int_{\mathbb{R}^n} \exp\left(-\widehat{\mathbf{x}}^T \widehat{\mathbf{x}} \right) \mathbf{p}\left(\sqrt{2}\mathbf{C}^{\frac{1}{2}}\widehat{\mathbf{x}} + \mathbf{m}\right) \, \left( 2^{\frac{d}{2}} \det(\mathbf{C})^{\frac{1}{2}}\right) \, d\widehat{\mathbf{x}} \\
% &= Z \, \pi^{-\frac{n}{2}} \int_{\mathbb{R}^n} \exp\left(-\widehat{\mathbf{x}}^T \widehat{\mathbf{x}} \right) \mathbf{p}\left(\sqrt{2}\mathbf{C}^{\frac{1}{2}}\widehat{\mathbf{x}} + \mathbf{m}\right) \, d\widehat{\mathbf{x}}.
% \end{split} \end{equation*}
% Applying Gauss-Hermite quadrature then provides the final result.
% \end{proof}
% \begin{remark}
% Note that in the above equations, the expressions for the shape parameters and normalizing coefficient of the product distribution for the random variable $\mathbf{X}$, i.e. $\mathbf{m},\,\mathbf{C},$ and $Z$, all depend on indices $i_1,\dots,i_\alpha;j_1,\dots,j_\beta$ even if not explicitly indexed.
% \end{remark}

% \subsection{Other Implementation Details}
% ~\\

% \JONAS{
% \begin{itemize}
% \item Optimizer either Adam or LBFGS (preferred), with coefficients in Gaussian basis linearly constrained to be solution of discretized problem (i.e. LSGD-style)
% \item Adam runs for either 1K or 10K steps with learning rate of $\lambda = 0.001$
% \item LBFGS runs for 100 or 500 steps with learning rate of $\lambda = 0.01$, with 5 substeps and a history of 16 steps, with tolerances of $1.0 \times 10^{-14}$
% \item Loss is Relative L2 for `standard form' problems or (non-relative) H1 for mixed form problems, computed via sampling at data sites
% \item Data is uniformly-chosen points inside interior of $\Gamma$, for $N=4096$ data points. Boundary data for collocation is also computed by sampling from uniformly-chosen random points on $\Gamma$
% \item Code run on 1 Nvidia a100 GPU (41GB) using PyTorch
% \end{itemize}
% }

%%%%%%%%% CUT AND PASTED %%%%%%%%%%%%%%%

\subsection{Consistency and Compatibility on Infinite Domains}
% \begin{itemize}
% \item no consistency error since no boundary term 
% \end{itemize}

Since our scheme is conforming when $~u\in H^1_c(\mathbb{R}^d)$, it is worth showing that the discretization we choose is consistent.  To that end, suppose $H^1_{0,h}(\mathbb{R}^d) \subset H^1_0(\mathbb{R}^d)$ is chosen based on a given ``mesh'' of RBFs, and let $~u_h\in H^1_{0,h}(\mathbb{R}^d)$ be the solution to $a(~u_h,~v_h) = f(~v_h)$ for all $~v_h\in H^1_{0,h}(\mathbb{R}^d)$.  Given a strong-form solution $~u\in C^2(\mathbb{R}^d)$, it follows that \ANT{stating this for Poisson, but conclusions apply more generally}   
\begin{align*}
    a(~u-~u_h,~v_h) = a(~u,~v_h) - f(~v_h) = -\int_{\mathbb{R}^d}\lr{\Delta~u+~f}\cdot~v_h = 0,
\end{align*}
where integration by parts was applied and we used that $~v_h\in H^1_0$.  Therefore, this scheme will be convergent provided it is also stable \ANT{Isn't this automatic from the Whitney form construction?  We should show it if so.}.

\subsection{Consistency and Compatibility on Bounded Domains}
\begin{itemize}
\item boundary penalty method $\rightarrow$ changes to bilinear form
\item MC sampling or quadrature on boundary; this is not so terrible even for high-dimensional problems, since the boundary is of a lower dimensions so sampling is less costly \\
\end{itemize}

% In practice, it is usually the case that the domain of interest $\Omega\subset\mathbb{R}^d$ for the PDE is bounded by a (regular enough) curve $\Gamma$, so that the finite element trial space $H^1_{0,h}(\mathbb{R}^d)$ is not contained in the space of solutions to $a(~u,~v) = f(~v)$, making our scheme nonconforming.  This creates issues for the enforcement of boundary conditions such as $~u|_{\Gamma} = ~g$, as it is not obvious how to enforce this condition essentially in the trial space.  To circumvent this issue, we apply Nitsche's method \cite{nitsche_stuff}, which is a modification of the boundary penalty method designed to remove the consistency error which is incurred by enlarging the finite element trial space to remove the strong boundary condition \ANT{should include some description of the method here}.

% On the other hand, since our trial space necessarily has global support, the crux of our method relies on using machine learning methods to minimize the inevitable consistency error which arises due to the approximation of integrals over the finite domain $\Omega$ with integrals over the infinite domain $\mathbb{R}^d$. While it is unfortunate that such error occurs in the first place, it is important to note that consistency error will only affect the convergence rate of the scheme, which is of minor concern since the method has been designed to be applied as a reduced model \ANT{should say this better}.  

% To understand what is happening, consider $\Omega\in\mathbb{R}^d$ and $~u,~v\in H^1(\Omega)$, and define
% \begin{align*}
%     a^{pen}(~u,~v) = \int_\Omega \nabla~u:\nabla~v + \gamma\int_\Gamma ~u\cdot~v, \\
%     f^{pen}(~u,~v) = \int_\Omega ~f\cdot~v + \int_\Gamma ~g\cdot~v,
% \end{align*}
% where $\gamma\in\mathbb{R}^+$ is a penalty parameter.
% It follows that solutions to $a^{pen}(~u_h,~v_h) = f^{pen}(~v_h)$ increasingly satisfy the boundary condition $~u|_{\Gamma}=~g$ as $\gamma\to\infty$, but this comes at the price of a consistency penalty:
% \begin{align*}
%     a^{pen}(~u-~u_h,~v_h) &= a^{pen}(~u,~v_h) - f^{pen}(~v_h) \\
%     &= \int_\Gamma \nabla_{~n}~u\cdot~v_h -\int_\Omega (\Delta~u + ~f)\cdot~v_h + \gamma\int_\Omega (~u-~g)\cdot~v_h \\
%     &= \int_\Gamma \nabla_{~n}~u\cdot~v_h \neq 0,
% \end{align*}
% since $~v_h$ is no longer zero on the boundary $\Gamma$.  This would not be a problem \textit{if we could compute integrals on $\Omega$}, since Nitsche's method defines the new bilinear form and linear functional
% \begin{align*}
%     a^N(~u,~v) &= \int_\Omega\nabla~u:\nabla~v + - \int_\Gamma \nabla_{~n}~u\cdot~v + \int_\Gamma\nabla_{~n}~v\cdot~u + \gamma\int_\Gamma ~u\cdot~v, \\
%     f^N(~v) &= \int_\Omega f\cdot~v + \int_\Gamma ~g\cdot~v.
% \end{align*}
% Here, the problem term has been added back into the bilinear form to eliminate the consistency penalty, and a symmetry term has been added to both $a^N,f^N$ in order to produce a symmetric bilinear form without changing the weak-form equations.  With these modifications, it is easy to check that $a^N(~u-~u_h,~v_h) = 0$, yielding a consistent repair to the penalty method from before.

% As mentioned, in our case we will use integrals on $\mathbb{R^d}$ as a surrogate for integrals on $\Omega$, which necessarily induces consistency error in the weak-form system.  Indeed, we restrict attention to $~u,~v\in H^1_0(\mathbb{R}^d)$ and define
% \begin{align*}
%     \bar{a}^p &= \int_{\mathbb{R}^d}\nabla~u:\nabla~v + \gamma\int_\Gamma ~u\cdot~v = a^p(~u,~v) + \int_{\Omega^c}\nabla~u:\nabla~v, \\
%     \bar{f}^p &= \int_{\mathbb{R}^d}\bar{~f}\cdot~v + \gamma\int_\Gamma ~g\cdot~v = f^p(~u,~v) + \int_{\Omega^c}\bar{~f}\cdot~v,
% \end{align*}
% for some predefined and regular enough extension $\bar{~f}$ of $~f$ which agrees with $~f$ on $\Omega$.  Defining $~u_h$ as the solution to $\bar{a}(~u_h,~v_h) = \bar{f}(~v_h)$, it follows as before that
% \begin{align*}
%     a(~u-~u_h,~v_h) 
% \end{align*}

% % \begin{align*}
% %     a(~u,~v) &= \int_\Omega \nabla~u:\nabla~v = \int_{\mathbb{R}^d} \nabla~u:\nabla~v - \int_{\Omega^c} \nabla~u:\nabla~v \coloneqq \bar{a}(~u,~v) - \int_{\Omega^c}\nabla~u:\nabla~v, \\
% %     f(~v) &= \int_\Omega ~f\cdot~v = \int_\mathbb{R}^d \bar{~f}\cdot~v - \int_{\Omega^c} \bar{~f}\cdot~v \coloneqq \bar{f}(~v) - \int_{\Omega^c} \bar{~f}\cdot~v,
% % \end{align*}
% % for some regular enough extension $\bar{~f}$ of $~f$ which agrees with $~f$ on $\Omega$.  

% Our goal will be to compare the original variational problem in terms of $a,f$ to its extension in terms of $\bar{a},\bar{f}$.
% %should mention BCs and penalty method?

% First, suppose $~u\in H^1_0(\mathbb{R}^d)$ and $~u_h, ~v_h\in H^1_{0,h}(\mathbb{R}^d)$ \ANT{need to define all these spaces}, then choosing $~u_h$ as the solution to $\bar{a}(~u_h,~v_h) = \bar{f}(~v_h)$, the consistency error in the discretization becomes
% \begin{align*}
%     a(~u-~u_h,~v_h) &= a(~u,~v_h) - \left(\bar{f}(~v_h) - \int_{\Omega^c}\nabla~u_h:\nabla~v_h\right) \\
%     &= \lr{a(~u,~v_h)-f(~v_h)} + \lr{\int_{\Omega^c}\nabla~u_h:\nabla~v_h - \int_{\Omega^c} \bar{~f}\cdot~v_h} \\
%     &= \int_{\Omega^c}\nabla~u_h:\nabla~v_h - \int_{\Omega^c} \bar{~f}\cdot~v_h \neq 0.
% \end{align*}
% Therefore, even when boundary conditions are enforced strongly, there is inconsistency in the scheme which depends on how the extension $\bar{~f}$ is chosen, as well as how much the mass of $~u_h$ is concentrated outside the effective domain $\Omega$.  The assumption we make is that this can be made sufficiently small with appropriate training.

\ANT{Are $H^1$ functions with trace vanishing on a zero-measure set dense in $H^1$?  I think yes}
